Visual tests using several safe confidence intervals

We propose a new statistical hypothesis testing framework which decides visually, using confidence intervals, whether the means of two samples are equal or if one is larger than the other. With our method, the user can at the same time visualize the confidence region of the means and do a test to decide if the means of the two populations are significantly different or not by looking whether the two confidence intervals overlap. To design this test we use confidence intervals constructed using e-variables, which provide a measure of evidence in hypothesis testing. We propose both a sequential test and a non-sequential test based on the overlap of confidence intervals and for each of these tests we give finite-time error bounds on the probabilities of error. We also illustrate the practicality of our method by applying it to the comparison of sequential learning algorithms.

==> intro.tex <==

\begin{abstract}%
We propose a new statistical hypothesis testing framework which decides visually using confidence intervals whether the means of two samples are equal or if one is larger than the other. With our method, the user can at the same time visualize the confidence region of the means and do a test to decide if they are significantly different or not by looking whether their confidence intervals overlap. To design this test we use confidence intervals constructed using e-variables and safe statistics techniques. We propose both a sequential test and a non-sequential test based on the overlap of confidence intervals and for each of these tests we give finite-time error bounds on the probabilities of error. We also illustrate the practicality of our method by applying it to the comparison of sequential learning algorithms.
\end{abstract}


\begin{keywords}%
Nonparametric statistics, E-values, Anytime confidence intervals%
\end{keywords}
\todoT{$n$ versus $m$. Careful cite vs citep. Careful of the ranges when not $1$, check homogeneity.}

\section{Introduction}


Confidence intervals on the mean are an important tool in descriptive statistics and are often used by practitioners to compare the means of several populations ``by eye'', i.e. deciding that the mean of two populations are different if and only if the confidence intervals are disjoint.
In theory, this comparison ought to be a test of hypothesis between the means, but deducing a pairwise test from confidence intervals on individual series of data can be tricky, this is the subject of this paper. 

We see two natural usages of such confidence intervals. One is in exploratory data analyses in which one may want to visually decide whether a certain feature is relevant to decide between two categories in a classification problem. A second usage is when comparing several machine learning algorithms. The results of such comparison can be several confidence intervals on the performances, one for each algorithm, and the plot of these confidence intervals can then be used to see quickly which of two algorithms is the best one and get information on the actual mean performance of each algorithm.

If we have two samples $X_1,\dots,X_n$ i.i.d. from a law $P$ and $Y_1,\dots,Y_m$ i.i.d. from a law $Q$, used to construct two confidence intervals $C_n(\alpha; X)$ and $C_m(\alpha;Y)$ such that $\P_P(\E_P[X] \in C_n(\alpha; X)) \ge 1-\alpha$ and $\P_Q(\E_Q[Y] \in C_m(\alpha;Y)) \ge 1-\alpha$ for some $\alpha \in (0,1)$, we are tempted to say that if the two confidence intervals $C_n(\alpha;X)$ and $C_m(\alpha;Y)$ do not overlap, then we can reject $H_0:\E_P[X] = \E_Q[Y]$ otherwise we do not reject $H_0$, we call this the test of overlap. It is easy to see that such a test has a type I error at most $2\alpha$ however it is known that the actual error of such test is often lower than $2\alpha$, and this asks the question of what is the actual type I error of this test. 

In the case of Gaussian random variables, this question has been answered in \cite{goldstein1995graphical} provided that the variances of $P$ and $Q$ are known. \textbf{Our main contribution} is to provide confidence intervals and associated visual tests of overlap, with theoretical guarantees in a nonparametric setting in which we suppose that the distributions are bounded. We provide both sequential and non-sequential test. We construct the confidence intervals using the betting principle~\citep{waudby2024estimating} and the notion of e-variables which can be seen as a notion of evidence, the higher the e-variable the less likely it is that $H_0$ is true. It is convenient to use e-variables because they can easily be combined and provide a natural interpretation as evidence in a test. We propose both anytime and fixed time results allowing for a sequential test in which the data come as a stream.

More precisely, let $X_1,X_2,\dots$ be i.i.d. from a law $P$  and $Y_1,Y_2,\dots$ be i.i.d. from a law $Q$ independents of $X_1,X_2,\dots$, with $P$ and $Q$ having bounded supports. In the sequential setting, we construct a sequence of anytime confidence intervals $\{C_n(\alpha;X)\}_n$ and $\{C_m(\alpha,Y)\}_m$, and in the non-sequential setting, we have access to a sample $X_1,\dots,X_n$ and a sample $Y_1,\dots,Y_n$ from which we construct two confidence intervals $C_n(\alpha;X)$ and $C_m(\alpha,Y)$.
Moreover, we construct a sequential and a non-sequential test of visual overlap to decide between the following three hypotheses
$$H_1^-: \E_P[X] < \E_Q[Y] - \Delta,\quad H_0 : \E_P[X] = \E_Q[Y], \quad H_1^+: \E_P[X] > \E_Q[Y] + \Delta,$$
for some effect size $\Delta>0$ assumed known in advance. For this test we show error bounds that are summarized in Table~\ref{table:errors} (see the Theorems~\ref{th:typeIerror},~\ref{th:typeII_anytime},~\ref{th:typeII_hoeffding},~\ref{th:typeIII} for the non-asymptotic error bounds). Remark that the three hypotheses can easily be reduced to the more usual bilateral test if needed.
\begin{figure}[h]
\begin{center}
\small
\begin{tabular}{ |p{2cm}||p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|  }
 \hline
 &\multicolumn{2}{|c|}{$\E_P[X] < \E_Q[Y] - \Delta$} & \multicolumn{2}{|c|}{$\E_P[X] = \E_Q[Y]$} & \multicolumn{2}{|c|}{$\E_P[X] > \E_Q[Y] +\Delta$} \\
 \hline
Sequential & Yes & No & Yes & No & Yes & No  \\
 \hline
\hline
Decide $H_1^-$    &  No error   &  No error   & $ \alpha$ & $ \alpha e^{-\Delta\Omega(\sqrt{n})}$& $2\alpha^2$ & $2\alpha^2$\\
 \hline
Decide $H_0$    &  $\alpha^{3/2}$   &  $\alpha^{3/2}$  & No error& No error& $\alpha^{3/2}$ & $\alpha^{3/2}$\\
 \hline
Decide $H_1^+$    &  $2\alpha^2$   &  $2\alpha^2$   & $ \alpha$ & $ \alpha e^{-\Delta\Omega(\sqrt{n})}$& No error & No error\\
 \hline
\end{tabular}
\end{center}
\caption{Approximate probabilities of error of the overlap test for $n$ sufficiently large (Fixed-time test) or  after decision (sequential test)\label{table:errors}}
\end{figure}


Finally, in Section~\ref{sec:xp} we showcase the practical efficiency and its usage in a task for exploratory data analysis and to compare the performance of some reinforcement learning agents.

\paragraph{Related works on tests from confidence intervals}
All previous works are in the Gaussian setting with known variance. The first work on this problem dates back to~\cite{goldstein1995graphical}, after which several applied papers~\citep{AUSTIN2002194,knol2011mis,schenker2001judging} have either proposed alternative methods or commentary on how to do visual tests using confidence intervals. to derive a test from confidence intervals, but always in the case of a Gaussian model with known variances.

\paragraph{Related works on nonparametric confidence intervals using E-variables}
E-values~\citep{10.1093/jrsssb/qkae011,ramdas2023game,ramdas2024hypothesis} are an alternative to p-values for tests. Their main advantages over p-value is that the bigger the e-value is, the more confidence we are that we should reject $H_0$, which means that e-values are a measure of \textbf{evidence}. Moreover, e-values are often \textbf{anytime-valid}, in other words they can deal with data that are collected sequentially. Of particular interest for our article, we will look at the technique leveraging e-values to construct confidence intervals introduced in \cite{waudby2024estimating} in the case of bounded random variables. 

